On single-point inversions of magnetic dipole lines in the corona

Prompted by a recent paper by Dima and Schad, we re-consider the problem of inferring magnetic properties of the corona using polarimetric observations of magnetic dipole (M1) lines. Dima and Schad point to a potential source of degeneracy in a formalism developed by Plowman, which under some circumstances can lead to the solution being under-determined. Here we clarify the nature of the problem. Its resolution lies in solving for the scattering geometry using the elongation of the observed region of the corona. We discuss some conceptual problems that arise when casting the problem for inversion in the observer's reference frame, and satisfactorily resolve difficulties identified by Plowman, Dima and Schad.

==> extras <==

In Plowman's method, the emission can arise 
from \textit{any} point (e.g., $P$ or  $P'$) in the figure, but
only some of these points will be compatible with the derived alignment factors  $\sigma_J$ and $\sigma_{J_0}$.   In essence,
without using embedded information contained from 
these alignment factors, one has no constraints on the LOS coordinate $x$.   One could explore as a function of 
$x$, for each observed  $y$-coordinate, those
solutions which are compatible with the derived solutions. \textbf{\emph{(This sentence sounds a bit ``circular''... I suggest to simplify this last two sentences as follows ``To overcome this limitation requires 
\textit{using another observable}, the $y$-coordinate.'' or something to that extent.}}
This new step 
requires 
\textit{using another observable}, the $y$-coordinate.  


$\hat{\mathbf b}$
The factors $C_{JJ_0}$ 
are common to each line. 
By taking observed and theoretical ratios $Q/I, U/I$ and $V/I$, we eliminate this variable, 
leaving just three observed ratios from which four unknowns are to be 
found.  


(\ref{eq:I}) to 
 (\ref{eq:V})
 
 \newcommand{\st}[]{\sin^2\Theta_B}
 \begin{equation}   
    \frac{V_1}{V_2} 
    =
    \frac{    
    {\bar{g}_{1}\lambda_{1}} (
    {I_1 \pm L_1}) +     \frac{2F_1 L_1
}{3\st^2}}{
{\bar{g}_{2}\lambda_{2}} (
    {I_2 \pm L_2}) +     \frac{2F_2 L_2
}{3\st^2}}
\end{equation}
 
 
 
 

\footnote{The ``single point'' approach replaces the integral of the emission coefficients (equations 35a-35c) along the line-of-sight direction by one average point multiplied by a characteristic length, avoiding an  intractable inverse problem 
\citep{Judge2007}, in which one might attempt to solve for quantities along the line-of-sight, in a fashion equivalent to emission measure analysis.  But this approach does not make sense when one is seeking to  measure the vector magnetic field 
{\bf{B(r)}} in the three-dimensional
volume of the corona, instead of a 
line-of-sight integrated quantity 
such as the emission measure. }.


Given more independent observables than
model parameters, an approach such as 
least-squares minimization would be 
appropriate.  However, in this particular problem, one of the eight equations is redundant, as can be seen from the analytic solution for the ``magnetic azimuth'' angle  $\gamma_B$:
\begin{equation} \label{eq:gammab}
    \gamma_B = - \frac{1}{2} \arctan \frac{U^{(i)}}{Q^{(i)}}, \ \ \ \mathrm{for\ both \ lines\ }(i)=1,2.
\end{equation}
In using equation~(\ref{eq:gammab})
with one or both lines, 
the number of independent measurements is reduced to seven, since one unknown is 

The figure also shows another 
angle $\vartheta_B$, undetermined by the 
analytical solution, 
and we have \citep{Casini+Judge1999}:
\begin{equation}
	\label{eq:cos}
\cos\Theta_B
	=\cos\vartheta\cos\vartheta_B+\sin\vartheta\sin\vartheta_B\cos\varphi_B\;,
\end{equation}
where another angle $\varphi_B$ is the angle between the normal to the planes containing $\mathbf{ \hat s}$ and $\mathbf{ \hat k}$,
and $\mathbf{ \hat s}$ and $\mathbf{ \hat b}$ respectively.  If we examine equation (\ref{eq:cos}) keeping the value of $\Theta_B$ fixed at a value from the analysis of 
\citet{Plowman_2014}, then 


Quantities 
Now $\vartheta$ 


Let us go further and 
look only at the parametric
dependencies on only $I^{(i)}$
and $L^{(i)}$, we have four observables depending on the following five parameters:
$$
\Theta_B, \ \ \mathrm{and}\  \  C^{(i)},  \sigma^{(i)}, 
\ \ i=1\ldots 2.
$$





Some research has   
studied the further possibility of
using  
only measurements of  $I,L$,  ($L^2 = Q^2+U^2$), in order to
attempt to recover all parameters except for $B$ and $\Theta_B$ from observations
$$
C^{(1)}, C^{(2)} ,\sigma^{(1)}, \sigma^{(2)}.
$$
In these studies, all hope of
finding the LOS field is abandoned, and the 


\subsection{Rescuing the Plowman formalism}




(\ref{eq:U}) and 
 (\ref{eq:Q})
 
 
The first idea of localized emission cannot be justified, but it may be a useful approximation for  structures such as
dense coronal loops in active regions, and polar plumes.  It is clear
that the same assumption 
is used implicitly in many studies of 
EUV intensity spectra and images of
the Sun, such as in the elementary thermal diagnoses of active region loops and in coronal seismology. 


In studying Plowman's application to the well-known \ion{Fe}{13}
line pair at 1074.7 and 1079.8 nm, \citet{Dima+2020} examined the  algebraic solutions to the problem posed by Plowman, uncovering an important error in an algebraic factor inherited from 
an incorrect formula in 
CJ99 (their expressions 37b and 38b). However, as 
shown by \citet{Dima+2020},
this error led to no 
fundamental problems in 
using Plowman's method. This issue will not be discussed 
further.



conditions where the pair 
of lines both satisfy 
the condition 
Clearly $F=0$ when $J=1,J_0=0$ and/or when $g_J=g_{J_0}$, where 
$g_J$ is the Land\'e g-factor for level $J$ 
($\ne \bar{g}_{JJ_0}$).
If we consider the 
line pair of M1 lines of
silicon-like \ion{Fe}{13}, then $F=0$
for the $J=1 \rightarrow J=0$ transition at 
1074.7 nm belonging to the $3p^2\,^3\!P$ ground term.
Under conditions of \textit{LS-coupling}, $F=0$ also
for the $J=2 \rightarrow J=1$ transition at 
1079.8 nm, because the LS coupled Land\'e factors are 
\begin{equation}
  g_J \simeq  \frac{3}{2} + \frac{S(S+1) - L(L+1)}{2J(J+1)},
\ \ \mathrm{for}\ J \ne 0,\label{eq:LScoupling}
\end{equation}
so that when $S=L$ 
(the case for the 
$3p^2\;^3\!P$ levels of \ion{Fe}{13}),
$g_J = g_{J_0}$ for 
both lines. 
This presents a potentially serious problem. 


 But first we
 re-examine the way that this problem has been posed.




\citep[see figure~\ref{fig:sphere}, discussed by e.g.,][]{Judge2007}, which is related to 
the angles $\Phi_B$ and $\Theta_B$ via 
\citep[eq. 44 or ][]{Casini+Judge1999}
\begin{equation*}
\sin\Theta_B\cos\Phi_B 
= \cos\vartheta\sin\vartheta_B\cos\phi_B - \sin\vartheta\cos\theta_B,
\end{equation*}
where all of the angles on the RHS of the equation, defined in the "S-frame", vary 
as $x$ varies




The algebraic solutions contain no explicit 
variables in the \textit{solar} rest frame,
in which at each point in
the plane-of-the-sky (POS), one must fix the coordinate along the LOS in order to
evaluate the emission
coefficients.  This is evidently the case when we consider two points P and P' along the LOS (Figure~\ref{fig:sphere}),
which have the same 
magnetic field vector 
 $\hat {\mathbf b}$.  The two points must have different polarizations owing to the 
quite different angle between the center of anisotropic irradiation (the solar center at point O) and $\hat {\mathbf b}$,
yet 


influence the foundations 
for the interpretation of 
Stokes forbidden line data 
acquired with  earlier
experiments such as the KELP 
\citep{Querfeld1977} 
and CoMP \citep{CoMP} instruments,  many  eclipse experiments
\citep[e.g.][]{Penn+Kuhn1994,Penn+others1994b, 2007ApJ...663..598H,2010ApJ...708.1650H,2013SoPh..285....9H,2018ApJ...859..155B,Samra2018,2019ApJ...877...10J,2019SoPh..294..166J,
2019ApJ...873L..25S} and they are gaining 
more importance with the advent of DKIST, COSMO and 
other upcoming projects.




Plowman studied the inverse problem of using two spectral lines with eight 
independent measurements of
$(I,Q,U,V)^T$, four for each line, to solve to   solve for eight quantities emitted by one representative point along the line-of-sight (LOS).   
In principle, from eight observables one might attempt to solve for eight 
model parameters.   However, as made explicit by \citet{Plowman_2014} 
(equations 9-15) and \citet{Dima+2020} (equations 11-15) there are only \textit{seven} explicit variables which have been solved for for each point
 in 
the plane-of-the-sky (POS):
$$
B,\Phi_B,\Theta_B,  C^{(1)}, C^{(2)} ,\sigma^{(1)}, \sigma^{(2)},
$$
where superscripts  $(1)$ and $(2)$ are convenient labels for any pair of lines used (the lines actually used by Plowman were those of 
[\ion{Fe}{13}] at 1074.7 and 1079.8 nm).  On the surface, it appears as if the problem is 
\textit{over-constrained}.  However, in effect there are only \textit{seven} model
parameters in this
formulation
\citep{Plowman_2014}, because 
 the magnetic ``azimuthal'' angle  $\Phi_B$ is 
\begin{equation} \label{eq:gammab}
    \Phi_B = - \frac{1}{2} \arctan \frac{U^{(i)}}{Q^{(i)}}, \ \ \ \mathrm{for\ both \ lines\ }(i)=1,2.
\end{equation}
A ratio of the observed $U/Q$ ratio for both lines  suffices to define $\Phi_B$.
No other simple combination of
equations (35a-35c) of 
\citet{Casini+Judge1999}
can be used to determine one, and 
just one, parameter in the same way. 

Thus, \citet{Plowman_2014} and \citet{Dima+2020} both 
studied direct solutions for the seven parameters from the seven independent measurements.   
What, then, is the problem concerning the scattering geometry (Figure~\ref{fig:sphere})?  Let us assume that, in spite of the large sensitivity to measurement uncertainties
identified by Plowman, these seven parameters have been determined algebraically from the measurements, subject to
the well-known ambiguities arising from native
symmetries.
Having solved for 
$\Phi_B$, we are left with  six observables
$$
I^{(i)}, L^{(i)}, V^{(i)},
\ \ i=1\ldots 2,
$$
where ${L^{(i)}}^2 = {Q^{(i)}}^2+{U^{(i)}}^2$, for each line, from which we wish to determine the six remaining model  parameters
$$
B,\Theta_B, \ \ \mathrm{and}\  \  C^{(i)},  \sigma^{(i)}, 
\ \ i=1\ldots 2.
$$
When found, these parameters are sufficient to recover the vector magnetic field ($B_x,B_y, B_z$), again to within the known ambiguities. 
The derived  parameters 
are all local variables  
at some (as yet undetermined) point P, with coordinates {\bf r} in the frame with the Sun at point O. The point P is not explicitly determined by Plowman's method, which therefore 
appears to raise a question
concerning the whole approach,
because for any magnetic 
field unit vector ${\mathbf {\hat b}}$, 
the derived values of $\Phi_B$ and $\Theta_B$ are the same no matter 
if the emitting point is at
P or P' in Figure~\ref{fig:sphere}!  The values derived for $\Phi_B$ and $\Theta_B$ are invariant relative to any displacement of 
$\mathbf{\hat b}$ along the line-of-sight.  

However, there are  \textit{implicit} properties hidden in the remaining 
parameters determined by 
Plowman's method, which are
$$
C^{(1)}, C^{(2)} ,\sigma^{(1)}, \sigma^{(2)}.
$$
The first two parameters are proportional to the populations of the upper levels, which have an implicit dependence on the plasma density $n$, and 
the total solar irradiation 
$J^0_0$
at point P.   The parameters $\sigma^{(i)}$ for the two 
lines are implicitly dependent on $n$, the 
radiation anisotropy
$J^2_0$, and the angle $\vartheta_B$ between $\hat{\mathbf b} $
and the unit vector $\hat{\mathbf s}$ to point P from Sun center (Figure~\ref{fig:sphere}). We can write:
\begin{eqnarray}
C^{(i)} &=& C^{(i)}\{n,J^0_0\}, \ \ \ i=1\ldots2\\
\sigma^{(i)} &=& \sigma^{(i)}\{n,J^2_0, \vartheta_B\} \ \ \ i=1\ldots2
\end{eqnarray}
where $\{p,q,\ldots\}$ denotes an \textit{implicit functional dependence} on 
parameters $p,q,\ldots$.  These relations couple the four derived quantities to the four variables $n,J^0_0,J^2_0, \vartheta_B$, which, again subject to degeneracies caused by symmetries, can be determined 
again using an implicit method.
Thus we can regard 
the variables $n,J^0_0,J^2_0, \vartheta_B$ as being determined once the $C^{(i)}$
and $\sigma^{(i)}$ are known.

Now, for each radial
distance ($r=|{\mathbf r}|$ from Sun center), 
the parameters $J^0_0,J^2_0$
can be computed as a function of $r$ given limb-darkening 
measurements of the irradiation at the line wavelengths.   In turn, we can then determine $r$ which, for a given observation at position
$y,z$ on the sky, yields the magnitude of the position along the line of sight, $x$.  

To conclude, 
the method of Plowman implicitly solves 
for the position $x$ of the emitting point P along the line of sight. The extra degree of freedom that appears to be 
present, is absent once 
the relationships between the
derived $C^{(i)}$ and $\sigma^{(i)}$, and the 
more elementary variables 
 $n,J^0_0,J^2_0, \vartheta_B $
 are studied in the solar frame of reference.

\subsection{Degeneracies}

\citet{Dima+2020} showed that Plowman's method will fail for some special cases 
because of embedded symmetries in the coefficients 
$D_{JJ_0}$ and $E_{JJ_0}$ under
conditions that 
appear to to common.  These symmetries were
absent in Plowman's calculations because of the error inherited by Plowman in adopting the  expressions (37b) and (38b)  for $E_{JJ_0}$ (the general expression (36c) of CJ99 is correct). The calculations for  \citet{Plowman_2014}
are qualitatively valid for spectral
line pairs which do not contain 
underlying 
symmetries identified by \citet{Dima+2020}.

Many of the strongest M1 coronal lines belong to the $np^2 \, ^3P$ ground terms
for the C- ($n=2$ and Si-like ($n=3 $) ions,  including  the 
two Si-like \ion{Fe}{13} lines).  Thus,  the list of 13 prominent lines compiled by \citet{Dima+2020}
contains 9 transitions of the type $np^2\, ^3P_J 
\rightarrow np^2\, ^3P_{J_0}$ for which 
$g_{J}=g_{J_0}$ in LS coupling, and no solution to the 
single-point inverse problem using pairs of such lines is possible.
  On this basis, \citet{Dima+2020} suggested combining  
ions of the 
N- and P- like 
isolectronic sequences (in particular N-like  \ion{Si}{10}) with 
those of the C- and Si-like ions. The table of \citet{Dima+2020}
omits ions of the O- and S- sequences whose energy levels in LS coupling are 
in reverse order 
($J=2$ being lowest
in energy), 
even though there are several lines of potential 
interest
(\citealp{Judge1998}), and for which line pairs would not suffer from
degeneracy of the first kind because 
the first term of
equation~(\ref{eq:Fdima}) is never zero. 

These issues have prompted us to study the departure of Land\'e g-factors of LS-coupling using large-scale atomic structure  calculations 
\citep{Schiffman+others2020}.   For the \ion{Fe}{13} calculations the g-factor of the $J=2\rightarrow 1$ transition differs by 2.7\%{} from the LS-coupled value.  This makes the use of the \ion{Fe}{13} line pair susceptible to small amounts of noise, using the single-point inversion scheme.   





In these cases 
 we have 
\begin{eqnarray}
    \label{eq:FJJ} \nonumber
    \frac{E_{J,J_0=J}}{D_{J,J_0=J}}&=&
    - \sqrt{2}\left (\overline g_{J,J_0=J} - \frac{3}{2}g_{J_0}\right ), \mathrm{\ and\ so}\\ \nonumber
    F_{J,J_0=J}&=& -3 \left( \overline g_{J,J_0=J}-g_{J_0}
\right) \equiv -\frac{3}{2} (g_J- g_{J_0})
\end{eqnarray}
where we used the general relation (\ref{eq:gbar}). This expression is clearly 
of the same form 
as equation~(\protect\ref{eq:Fexpanded}) for $J=J_0$.





 While the omission of wavelengths by \citet{Dima+2020} is not a serious problem for ions  with lines 
where $\lambda_1\approx \lambda_2$, such as the important \ion{Fe}{13} pair at 1.0474 and 1.0798 $\mu$m, such a condition
is uncommon. For example, 
in the sulfur-like ions 
\ion{Fe}{11} and 
\ion{Ni}{13} the wavelength pairs  are 
0.7894 and 6.08, and 
0.51 and 19.3 $\mu$m respectively \citep{Judge1998}.

